Automated and Complete Generation of Traffic Scenarios at Road Junctions Using a Multi-level Danger Definition

To ensure their safe use, autonomous vehicles (AVs) must meet rigorous certification criteria that involve executing maneuvers safely within (arbitrary) scenarios where other actors perform their intended maneuvers. For that purpose, existing scenario generation approaches optimize search to derive scenarios with high probability of dangerous situations. In this paper, we hypothesize that at road junctions, potential danger predominantly arises from overlapping paths of individual actors carrying out their designated high-level maneuvers. As a step towards AV certification, we propose an approach to derive a complete set of (potentially dangerous) abstract scenarios at any given road junction, i.e. all permutations of overlapping abstract paths assigned to actors (including the AV) for a given set of possible abstract paths. From these abstract scenarios, we derive exact paths that actors must follow to guide simulation-based testing towards potential collisions. We conduct extensive experiments to evaluate the behavior of a state-of-the-art learning-based AV controller on scenarios generated over two realistic road junctions with increasing number of external actors. Results show that the AV-under-test is involved in increasing percentages of unsafe behaviors in simulation, which vary according to functional- and logical-level scenario properties.

==> chp/5-rw-table.tex <==
\newcommand{\colwidth}{0.8em}
\begin{figure}[tb]
	\centering
	\footnotesize
% 	\noindent
	\setlength{\tabcolsep}{4pt}
	%\hspace{-0.5cm}
	%\begin{tabular}{ m{2.2cm} c c c c c }
	%%%%%%%%%%%%%%%%%%%%%
% 	scenario Spec Languages
    \begin{subfigure}[b]{\columnwidth}
    \centering
    	\begin{tabular}{ l@{}l c c c c c c }
    		&& \rot[45][\colwidth]{Expressive}
    		& \rot[45][\colwidth]{Extensible}
    		& \rot[45][\colwidth]{Temporal}
    		& \rot[45][\colwidth]{Err. det.}
    		& \rot[45][\colwidth]{Concret.}
            & \rot[45][\colwidth]{Danger.} \\
    	%\end{tabular}
    	%\begin{tabular}{ l c c c c c }
    		\toprule
    		Ont.s \& models &\citep{Geyer2014,Klueck2018,Bagschik2018}
    		& \yes & \yes & \yes & \no   & \no  & \no  \\
    		Temporal scen.s &\citep{Queiroz2019GeoScenarioAn,Schutt2020,Hempen2017}
    		& \maybe  & \maybe    & \yes   & \no & \maybe   & \no \\
    		Gener. appr.s &\citep{Abdessalem2018TestingFeatureInteractionsBriandNsgaForConcreteScenes,Majumdar2021ParacsmJournal,Althoff2018}
            & \no   & \no   & \maybe & \no   & \yes    & \no\\
    % 		\midrule
    		\scenic &\citep{Fremont2019ScenicLanguage}
    		& \maybe   & \maybe   & \yes & \no   & \yes    & \no\\
    		\midrule
    		Our approach      &  & \yes   & \yes   & \no & \yes   & \yes    & \yes\\
    		\bottomrule
    	\end{tabular}
    % 	\hspace{0.5cm}
	\caption{Comparison of \textit{abstract scenario specification languages}}
	\label{tab:comparison-lang}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%
	scenario Spec Languages
    \begin{subfigure}[b]{\columnwidth}
    \centering
    	\begin{tabular}{ l@{}l c c c c }
    		&& \rot[45][\colwidth]{Arbitrary scen.}
    		& \rot[45][\colwidth]{Adj. num. cons.}
    		& \rot[45][\colwidth]{Map as input}
    		& \rot[45][\colwidth]{Grace. degr.} \\
    	%\end{tabular}
    	%\begin{tabular}{ l c c c c c }
    		\toprule
    		Search-based &
    		\citep{Abdessalem2018TestingFeatureInteractionsBriandNsgaForConcreteScenes,Babikian2021dReal,Wu2021} &
    		\maybe & \no & \no & \yes \\
    		Sampling-based &
    		\citep{Majumdar2021ParacsmJournal,Rocklage2018AutomatedScenarioGeneration,OKelly2018ScalableEndToEnd} &
    		 \maybe  & \maybe    & \no   & \no \\
    		Path Planning &
    		\citep{Althoff2018,Klischat2019} &
    		 \no   & \maybe   & \maybe & \no \\
    % 		\midrule
    		\scenic &      
    		\citep{Fremont2019ScenicLanguage} &
    		 \yes   & \maybe   & \yes & \no \\
    		\midrule
    		Our approach &         & \yes   & \yes   & \yes & \yes \\
    		\bottomrule
    	\end{tabular}\hspace{0.5cm}
    \caption{Comparison of \textit{scenario concretization approaches}}
	\label{tab:comparison-gen}
    \end{subfigure}
 
    \begin{subfigure}[b]{\columnwidth}
    \centering
    	\begin{tabular}{ l@{}l c c c }
    		&& \rot[45][\colwidth]{Arbitrary scen.}
    		& \rot[45][\colwidth]{Adj. num. cons.}
    		& \rot[45][\colwidth]{Map as input} \\
    	%\end{tabular}
    	%\begin{tabular}{ l c c c c c }
    		\toprule
    		Search-based &
    		\citep{Abdessalem2018TestingFeatureInteractionsBriandNsgaForConcreteScenes,Babikian2021dReal,Wu2021} &
    		\maybe & \no & \no \\
    		Sampling-based &
    		\citep{Majumdar2021ParacsmJournal,Rocklage2018AutomatedScenarioGeneration,OKelly2018ScalableEndToEnd} &
    		 \maybe  & \maybe    & \no \\
    		Path Planning &
    		\citep{Althoff2018,Klischat2019} &
    		 \no   & \maybe   & \maybe \\
    % 		\midrule
    		\scenic &      
    		\citep{Fremont2019ScenicLanguage} &
    		 \yes   & \maybe   & \yes \\
    		\midrule
    		Our approach &         & \yes   & \yes   & \yes  \\
    		\bottomrule
    	\end{tabular}\hspace{0.5cm}
    \caption{Comparison of \textit{scenario generation approaches}}
	\label{tab:comparison-gen}
    \end{subfigure}
    % Notation -- \yes: yes, \maybe: to a certain extent, \no: no.
    \captionsetup{justification=centering}
	\caption{Comparison of our approach with the existing state of the art. Notation -- \yes: yes, \maybe: to an extent, \no: no. }
	\label{tab:comparison-both}
	
    %%%%%%%%%%%%%%%%%%%%%
% 	scenario Spec Languages
    \begin{subfigure}[b]{\columnwidth}
    \centering
    	\begin{tabular}{ l l c c c c }
    		& & \rot[30][\colwidth]{Arbitrary scen.}
    		& \rot[30][\colwidth]{Adj. num. cons.}
    		& \rot[30][\colwidth]{Map as input}
    		& \rot[30][\colwidth]{Grace. degr.} \\
    	%\end{tabular}
    	%\begin{tabular}{ l c c c c c }
    		\midrule
    		Search-based        &
    		\citep{Abdessalem2018TestingFeatureInteractionsBriandNsgaForConcreteScenes,Babikian2021dReal,Wu2021} &
    		\maybe & \no & \no & \yes \\
    		Sampling-based      &
    		\citep{Majumdar2021ParacsmJournal,Rocklage2018AutomatedScenarioGeneration,OKelly2018ScalableEndToEnd} &
    		 \maybe  & \maybe    & \no   & \no \\
    		Path Planning       &
    		\citep{Althoff2018,Klischat2019} &
    		 \no   & \maybe   & \maybe & \no \\
    		\midrule
    		\scenic             &
    		\citep{Fremont2019ScenicLanguage} &
    		 \yes   & \maybe   & \yes & \no \\
    		\hline
    		Our approach        & \yes   & \yes   & \yes & \yes \\
    		\bottomrule
    	\end{tabular}\hspace{0.5cm}
    \caption{Comparison of \textit{scenario concretization approaches}}
	\label{tab:comparison-gen}
    \end{subfigure}
    % Notation -- \yes: yes, \maybe: to a certain extent, \no: no.
	\caption{Comparison of our approach with the existing state of the art. Notation -- \yes: yes, \maybe: to an extent, \no: no. }
	\label{tab:comparison-both}
\end{figure}

==> chp/7-biographies.tex <==

\newpage
\section*{Vitae}


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/bio/aren.jpg}}]
\textbf{Aren A. Babikian}
is a postdoctoral fellow in the Department of Computer Science at the University of Toronto
% PhD student at the Department of Electrical and Computer Engineering at McGill University.
His research focuses on using model generation techniques for the safety assurance of automotive systems, namely, autonomous vehicles.
He has published a related research paper at the international FASE conference (2020), as well as in the SOSYM (2021) and TSE (2024) journals.
He has also done related internships at NVIDIA and at AWS.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/bio/attila.jpg}}]
\textbf{Attila Ficsor}
received the Computer Science Engineer degree from the Budapest University of Technology and Economics in 2022. He is currently pursuing a PhD degree with the Critical Systems Research Group. His current research interests include model-driven engineering, graph transformation, and autonomous vehicle testing.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/bio/oszkar.jpg}}]
\textbf{Oszk\'{a}r Semer\'{a}th}
is an assistant professor at Budapest University of Technology and Economics. His research focuses on modeling technologies and logic solvers.
%He is the lead developer of the VIATRA Solver framework.
He won IEEE/ACM best paper award at \mbox{MODELS} conference, Young Researcher Award from the National Academy of Science, John George Kemeny Award from John von Neumann Computer Socienty, Amazon Research Award, and the New National Excellence Program scholarship three times.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/bio/gunter.jpg}}]
\textbf{Gunter Mussbacher}
is an associate professor at McGill University. His research interests include model-driven requirements engineering, software language engineering, next-generation reuse frameworks, sustainability, and human values. He holds a Ph.D. in Computer Science from the University of Ottawa, Canada. He serves on the editorial board of the Requirements Engineering journal and served as Program Co-Chair of RE 2022 and General Co-Chair of ICT4S 2023.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/bio/daniel.jpg}}]
\textbf{D\'{a}niel Varr\'{o}}
is a full professor at Linköping University and an adjunct professor at McGill University.  He is a co-author of 180+ papers with seven Distinguished Paper Awards, and three Most Influential Paper Awards. He serves on the editorial board of Software and Systems Modeling, and served as a program co-chair of MODELS'21, SLE'16, FASE'13 conferences. 
%He delivered keynote talks at numerous conferences (incl. CSMR, SOFSEM and SAM) and international summer schools. 
He is a co-founder of the VIATRA open-source transformation framework, and IncQuery Labs, a technology-intensive company.
% \end{IEEEbiography}

